Arrival-Intensity Control for A Single-Server Queue in Heavy Traffic

We study a single-server queue control problem (QCP) in a heavy-traffic regime, extending the framework from Lee and Weerasinghe (2011). The state process represents the offered waiting time. Service times and patience times form independent i.i.d. sequences with general distributions. We formulate an infinite-horizon discounted QCP that balances the cost of controlling the arrival intensity against a penalty for server idleness. A distinctive feature of the formulation is the nonstandard decreasing operational running cost arising from the arrival-intensity control mechanism. Under suitable heavy-traffic assumptions, the diffusion-scaled offered waiting-time process converges to a regulated diffusion, leading to an associated diffusion control problem (DCP). We find the optimal control of the associated DCP by incorporating the Legendre-Fenchel transform and a formal Hamilton-Jacobi-Bellman (HJB) equation. We then construct a sequence of intensity controls for the prelimit queueing systems from the DCP-optimal feedback and establish its asymptotic optimality within the specified heavy-traffic admissible control class. Beyond theoretical analysis, numerical experiments further examine whether reinforcement learning can approximate the optimal policy with discounted costs close to the HJB reference. Policies are trained from simulated state transitions and realized costs, and are evaluated against the independently computed HJB feedback.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


